CancerGPT: Few-shot Drug Pair Synergy Prediction using Large Pre-trained Language Models

Large pre-trained language models (LLMs) have been shown to have significant potential in few-shot learning across various fields, even with minimal training data. However, their ability to generalize to unseen tasks in more complex fields, such as biology, has yet to be fully evaluated. LLMs can offer a promising alternative approach for biological inference, particularly in cases where structured data and sample size are limited, by extracting prior knowledge from text corpora. Our proposed few-shot learning approach uses LLMs to predict the synergy of drug pairs in rare tissues that lack structured data and features. Our experiments, which involved seven rare tissues from different cancer types, demonstrated that the LLM-based prediction model achieved significant accuracy with very few or zero samples. Our proposed model, the CancerGPT (with $\sim$ 124M parameters), was even comparable to the larger fine-tuned GPT-3 model (with $\sim$ 175B parameters). Our research is the first to tackle drug pair synergy prediction in rare tissues with limited data. We are also the first to utilize an LLM-based prediction model for biological reaction prediction tasks.

==> tables/bone.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrrrr}\toprule
&\multicolumn{7}{c}{Predicted} \\\cmidrule{2-8}
\multirowcell{8}{Ground truth} & &\multicolumn{3}{c}{Synergy} &\multicolumn{3}{c}{No Synergy} \\\midrule
&\multirowcell{2}{Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Romidepsin, Thapsigargin, EW-8) \\ (Daporinad, Panobinostat, TC-32)}} &\multicolumn{3}{c}{\multirowcell{2}{(Carfilzomib, Entinostat, TC-32) \\ (Mocetinostat, Carfilzomib, TC-71)}} \\
& & & & & & & \\ \\
&\multirowcell{2}{No Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Thapsigargin, Beta-Narcotine, TC-32) \\ (SCHEMBL82368, Olaparib, TC-71)}} &\multicolumn{3}{c}{\multirowcell{2}{(Ethyl bromopyruvate, 717906-29-1, A-673) \\ (Doxorubicin Hydrochloride, Olaparib, TC-71)}} \\
& & & & & & & \\
\bottomrule
\end{tabular}
\caption{Example of prediction in bone tissue}
\label{tab:bone}
\end{table}

==> tables/liver.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrrrr}\toprule
&\multicolumn{7}{c}{Predicted} \\\cmidrule{2-8}
\multirowcell{8}{Ground truth} & &\multicolumn{3}{c}{Synergy} &\multicolumn{3}{c}{No Synergy} \\\midrule
&\multirowcell{2}{Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Piperacetazine, Aripiprazole, Huh-7) \\ (Idrocilamide, Sertraline hydrochloride, Huh-7)}} &\multicolumn{3}{c}{\multirowcell{2}{(3-Deazaneplanocin, Piperacetazine, Huh-7) \\
(Bepridil, Sertraline hydrochloride, Huh-7)}} \\
& & & & & & & \\ \\
&\multirowcell{2}{No Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Toremifene Citrate, Aripiprazole, Huh-7) \\ (Idrocilamide, Clomifene citrate, Huh-7)}} &\multicolumn{3}{c}{\multirowcell{2}{(Clomiphene, Mycophenolate Mofetil, Huh-7) \\
(3-Deazaneplanocin, Colchicine, Huh-7)}} \\
& & & & & & & \\
\bottomrule
\end{tabular}
\caption{Example of prediction in liver tissue}
\label{tab:liver}
\end{table}

==> tables/soft_tissue.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
&\multicolumn{7}{c}{Predicted} \\\cmidrule{2-8}
\multirowcell{8}{Ground truth} & &\multicolumn{3}{c}{Synergy} &\multicolumn{3}{c}{No Synergy} \\\midrule
&\multirowcell{2}{Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(915019-65-7, Trametinib, SMS-CTR) \\ (Omipalisib, Trametinib, RD)}} &\multicolumn{3}{c}{\multirowcell{2}{(Omipalisib, ceritinib, RD) \\
(SCHEMBL82368, Niraparib, Rh36)}} \\
& & & & & & & \\ \\
&\multirowcell{2}{No Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(BMS-754807, MK-2206, SMS-CTR) \\ (MK-1775, 955-24-8, Rh36)}} &\multicolumn{3}{c}{\multirowcell{2}{(Stattic, SU11274, DDLS8817) \\
(Akt inhibitor VIII, Stattic, DDLS8817)}} \\
& & & & & & & \\
\bottomrule
\end{tabular}
\caption{Example of prediction in soft tissue}
\label{tab:soft_tissue}
\end{table}

==> tables/stomach.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrrrr}\toprule
&\multicolumn{7}{c}{Predicted} \\\cmidrule{2-8}
\multirowcell{8}{Ground truth} & &\multicolumn{3}{c}{Synergy} &\multicolumn{3}{c}{No Synergy} \\\midrule
&\multirowcell{2}{Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Akt inhibitor VIII, Doramapimod, AGS) \\ (Doramapimod, SF1670, AGS)}} &\multicolumn{3}{c}{\multirowcell{2}{(5Z-7-Oxozeaenol, 10058-F4, AGS) \\
(5Z-7-Oxozeaenol, BI605906, AGS)}} \\
& & & & & & & \\ \\
&\multirowcell{2}{No Synergy} &\multicolumn{3}{c}{\multirowcell{2}{(Akt inhibitor VIII, SF1670, AGS) \\ (PI-103, SF1670, AGS)}} &\multicolumn{3}{c}{\multirowcell{2}{(CHIR-99021, GSK429286A, AGS) \\
(BI605906, 10058-F4, AGS)}} \\
& & & & & & & \\
\bottomrule
\end{tabular}
\caption{Example of prediction in stomach tissue (Drug A, Drug B, Cell line)}
\label{tab:stomach}
\end{table}
